Mean field dynamo action in shearing flows. II: fluctuating kinetic helicity with zero mean

Here we explore the role of temporal fluctuations in kinetic helicity on the generation of large-scale magnetic fields in presence of a background linear shear flow. Key techniques involved here are same as in our earlier work \citep[][hereafter paper~I]{JS20}, where we have used the renovating flow based model with shearing waves. Both, the velocity and the helicity fields, are treated as stochastic variables with finite correlation times, $\tau$ and $\tau_h$, respectively. Growing solutions are obtained when $\tau_h > \tau$, even when this time-scale separation, characterised by $m=\tau_h/\tau$, remains below the threshold for causing the turbulent diffusion to turn negative. In regimes when turbulent diffusion remains positive, and $\tau$ is on the order of eddy turnover time $T$, the axisymmetric modes display non-monotonic behaviour with shear rate $S$: both, the growth rate $\gamma$ and the wavenumber $k_\ast$ corresponding to the fastest growing mode, first increase, reach a maximum and then decrease with $|S|$, with $k_\ast$ being always smaller than eddy-wavenumber, thus boosting growth of magnetic fields at large length scales. The cycle period $P_{\rm cyc}$ of growing dynamo wave is inversely proportional to $|S|$ at small shear, exactly as in the fixed kinetic helicity case of paper~I. This dependence becomes shallower at larger shear. Interestingly enough, various curves corresponding to different choices of $m$ collapse on top of each other in a plot of $m P_{\rm cyc}$ with $|S|$.

==> removed.tex <==
NS: move the unused text/material to this file

There were few candidates to explain the dynamo in non-helical turbulence: shear-current effect \cite{kleeorin2003,RK08}, incoherent alpha effect \cite{VB97} and large-scale dynamo (LSD) due to suppression of small-scale dynamo (SSD) by shear \citep{TC13}. The first two effects are kinematic and the last one is non-linear dynamo mechanism. Many authors and simulations have shown the sign of relevant transport coefficient is not favourable for the shear-current effect \citep{RK06,BRRK08, SS09b,SS11}. \cite{You08a} have shown that the shear dynamo operates well below and above the threshold of fluctuation dynamo, indicating the underlying mechanism has to be kinematic in nature. 

 %NS: suppressing the following whole para as it doesn't seem necessary here
 %An important recognition is made by us in all studies \citep{RK08, HMS11,MB12,RP12}, which dealt with temporal $\alpha-$fluctuations, that the assumption of local interaction of magnetic field were imposed on the mean-field theory while deriving the evolution equation for magnetic field. Even though the original induction equation is non-local in magnetic field interaction. Even the work carried out in \cite{JNS18}, is for finite correlated $\alpha$-fluctuations (taking memory effect into account), we had considered the slowly varying magnetic field to reduce integro-differential equation for mean-field into PDE. The assumption of slowly varying mean field is again an assumption of local interaction of magnetic field with $\alpha$-fluctuations. Therefore, we have missed to capture the growth of first moment of magnetic field for pure temporal $\alpha-$fluctuations. The assumption of local interaction in turbulence date backs atleast to \cite{K41}; and in dynamos, it date backs to \cite{SKR66,KR80}, therefore it is difficult to break away from such a legacy. Recently, the importance of non-locality in the high magnetic Reynolds system is shown by number of studies \citep{CHT06,HY08,RB12}, where authors have shown that definition of the transport co-efficients ($\alpha$ and $\eta_t$) becomes ambiguous \citep{Hu08,CH09}. Even the usual objection to LSD due to the growing strength of small-scale fields in high Rm systems can be mitigated with the consideration of non-locality \citep{RB12}.
 
 
 
 A less common approach to study the dynamo is renovating flow models, where finite correlation of velocity field is naturally incorporated. In this model, time is spilt into the equal intervals of length $\tau$ and velocity field is assumed to be randomly and  independently distributed over the successive intervals drawn from the underlying probability distribution (PDF). Even though, such models lacks the continuous translational symmetry in time, it posses discrete translational symmetry in time $n\tau$: $n=0,1,2\dots$ and can be stationary as $n\to\infty$.  It is shown such model can give rise to fast dynamo representing the dynamo at high magnetic Reynolds number. \cite{GB92} considered the single scale helical flows in such a model and showed analytically the growing solution for the first moment of the magnetic field. \cite{KSS12} extended the GB92 model to include the linear shear and showed that there is no dynamo action if the flow is strictly non-helical. In \blue{Jingade \& Singh 2020} (paper~I), we showed the non-monotonic nature of the growth rate w.r.t shear in the helical flows, where the effect of shear is self-consistently considered in the amplitudes of the velocity field.
 
 
\cite{Kra76} has argued that the local helicity fluctuations whose mean helicity is zero in turbulence can give rise to anomalous magnetic diffusivity. When the helicity fluctuations having correlation time is longer than velocity correlation time, one can employ the double-averaging scheme. Initially, mean-field is obtained by averaging over the turbulent time scale and later again average this mean equation over the fluctuation time scale of the helicity to get the final mean-field equation and it was shown this helicity fluctuations tend to decrease the net magnetic diffusion (see \Eq{kraich_disper}) and if sufficiently strong can trigger dynamo due to negative diffusion. Note that, the origin of fluctuations in \cite{Hoy88} is fundamentally different from \cite{Kra76}   

\red{The reason being that, it is only the shear that appears in the magnetic evolution equation.}

%NS: moved the last para of discussion to here
%NS: it doesn't seem needed; only breaking the flow
 This idea of fluctuations has seem to motivated number of numerical techniques such as test field methods \citep{BRRK08}, singular-value decomposition method \citep{AbSu19} to measure the fluctuations in the averaged transport co-efficients in simulations and such measurements are further compounded by the difficulty due to non-local effects at high $\rem$ \citep{CH09,CA16} and tensorial $\alpha$-fluctuations, where linear relation between EMF and mean-field is replaced by linear integral relation \citep{HY08}. This seems to us is a hopeless attempt to come to the resolution of shear dynamo problem. Whereas, measurement of helicity correlation time and comparing with velocity correlation time is a more admissible task, which we hope to see in the near future.  


The question is when can there be a time scale separation between such fluctuations. We are beginning to realise that the non-normal turbulence that Kraichnan referred indeed could be the anisotropic turbulence naturally occurring in the shearing systems (also true in the presence of rotation and stratification), where inverse cascade of energy exist and can induce the time scale separation between various fluctuating quantities. This is our assertion and it needs to varied in the future simulation works. 


t would be a meaningful exercise to compare the correlation time of velocity and helicity in the background of rotating and shearing flows. 

%NS: this para below seems ok for thesis but not for the paper
%NS: so commenting this out

\begin{comment}
In the light of previously mentioned development, it is imperative to carry out correlation time measurements of helicity and velocity in rotating and shearing turbulence. Since, we had used single scale flow in the renovating flow model, the helicity that is associated is also of a particular scale. Even if the helicity correlation time is more than velocity correlation time in some range of scales, it can trigger the instability to generate the magnetic field according to the work carried out in this paper. It is a common knowledge in turbulence flows that correlation times are function of scales, therefore if for some scale $\tau_h(k)>\tau_u(k)$, where $\tau_u(k)$ and $\tau_h(k)$ are velocity and helicity correlation time as a function of scale, it is sufficient to trigger the dynamo according to the work presented here. As it is shown in recent works \citep{Sh18} that large scale vortex structures are developed due to inverse cascade of the energy in forced rotating turbulence, and it is observed that the two large vortex columns with opposite polarity appear with $80\%$ of fluid energy in them and rest $20\%$ is distributed in other modes of the field \citep{DS18}. If the fluid element enter into such vortex column with some angle to the column length (and this can happen due to randomness in the system), naturally this fluid element becomes helical. Since, there is two vortex column with opposite polarity, random entry of fluid element in to the column induces a fluctuations in the helicity at the scale of the vortex. Therefore, it seems promising to undertake the time scale separation measurement between helicity fluctuations and velocity fluctuations.
\end{comment}


\begin{comment}
In our work, we have not justified our assumption of helicity correlation
time to be more than the velocity correlation time. We have seen that the
shear plays quite a passive role by just amplifying the field, whose cause
of generation is helicity fluctuation. One can ask a question: Does shear
has a role in increasing the correlation time of helicity as compared to
velocity correlation time? One can make an attempt to answer that question
at-least in low Re regime, if one follows the work of the authors
\cite{SS10,SS11}, where they have derived the exact form of velocity
field satisfying Navier-Stokes equation without Lorentz term in low Re
limit. To check the correlation time of helicity, one has to construct
a quantity like $\langle h(\bsy{X},\tau)h(\bsy{X}',\tau')\rangle$ which
requires a four-point velocity correlator. It would be interesting to
construct such quantity and check whether indeed helicity correlation
time is more than velocity correlation or not.
\end{comment}


\begin{comment}
As we have seen in this section (\blue{give reference}), the first component (component in the direction of $X_1$) of the turbulent velocity field $\bfu$ is sheared out by the mean flow given by $SX_1\ey$. The question we are interested now is, can we extend the anti-dynamo theorem of Zeldovich to the velocity field $\bfu = (0,u_2,u_3)$, where $u_2=u_2(x_1,x_2,x_3)$, in the background shear flow? 
The induction equation with the background shear flow is given by
\beq
\left(\frac{\partial}{\partial t} + SX_1\frac{\partial }{\partial X_2}\right)\bfB +(\bfu\cendot\bnabla)\bfB-S\,B_1 \ey = (\bfB\cendot\bnabla)\bfu + \eta\nabla^2 \bfB
\eeq
The equation for the $B_1$ component is separated out 
\beq
\left(\frac{\partial}{\partial t} + SX_1\frac{\partial }{\partial X_2}\right)B_1 +(\bfu\cendot\bnabla)B_1 =  \eta\nabla^2 B_1
\label{b1_eqn}
\eeq
 This equation \ref{b1_eqn} resembles the advection-diffusion equation for the scalar. If we assume that the magnetic field vanishes at infinity, we can write the above equation as
 \beq
 \frac{\ud}{\ud t}\int_V B_1^2\, \ud V = -\eta \int_V (\bnabla B_1)^2\, \ud V
 \eeq
When $\eta=0$, we will have neither growth or decay of the magnetic field, the initial value remains. When $\eta>0$, then we will have exponential decay of the first component of the magnetic field. If we introduce the vector potential $\bfA$ as $\bfB = \bnabla\cross\bfA$, the $A_2$ and $A_3$ components goes to zero when $B_1=0$ for finite $\eta$. The equation obeyed by the $A_1$ component would be 
\beq
\left(\frac{\partial}{\partial t} + SX_1\frac{\partial }{\partial X_2}\right)A_1 +(\bfu\cendot\bnabla)A_1 =  \eta\nabla^2 A_1
\eeq
 The governing equation for $A_1$ is similar to the component $B_1$ and hence decays with time. If there is no growth in the single realisation of the field, there will not be growth even in the ensemble averaged mean-field. The strong shear makes the flow quasi-two dimensional and hence magnetic field decays in such a flow. One can workout in detail the nature of the decay and the rate of the decay as in \cite{Kol17} for the above mentioned flow. It would be an interesting exercise to carry out such a analysis.   
\end{comment}

